Toward Cognitive and Immersive Systems: Experiments in a Cognitive Microworld

As computational power has continued to increase, and sensors have become more accurate, the corresponding advent of systems that are at once cognitive and immersive has arrived. These \textit{cognitive and immersive systems} (CAISs) fall squarely into the intersection of AI with HCI/HRI: such systems interact with and assist the human agents that enter them, in no small part because such systems are infused with AI able to understand and reason about these humans and their knowledge, beliefs, goals, communications, plans, etc. We herein explain our approach to engineering CAISs. We emphasize the capacity of a CAIS to develop and reason over a `theory of the mind' of its human partners. This capacity entails that the AI in question has a sophisticated model of the beliefs, knowledge, goals, desires, emotions, etc.\ of these humans. To accomplish this engineering, a formal framework of very high expressivity is needed. In our case, this framework is a \textit{cognitive event calculus}, a particular kind of quantified multi-operator modal logic, and a matching high-expressivity automated reasoner and planner. To explain, advance, and to a degree validate our approach, we show that a calculus of this type satisfies a set of formal requirements, and can enable a CAIS to understand a psychologically tricky scenario couched in what we call the \textit{cognitive polysolid framework} (CPF). We also formally show that a room that satisfies these requirements can have a useful property we term \emph{expectation of usefulness}. CPF, a sub-class of \textit{cognitive microworlds}, includes machinery able to represent and plan over not merely blocks and actions (such as seen in the primitive `blocks worlds' of old), but also over agents and their mental attitudes about both other agents and inanimate objects.

==> past_and_future_models.tex <==
\subsection{Task 2 - Catching People Up}

The second task we define for our system is in assisting people
catch-up when they return to the room. As previously seen, we know
that $\humanb$ has missed that the goals of the room have changed, but
would perceive the new configuration of blocks. Thus, similar to the
previous task, he knows the location of the blocks and which are
clear, but does not know that the goals have changed.

However, sensing that something is amiss with the configuration per
his believed goal, the agent should be able to query the system as to
what has changed in the room while he was not in it, receiving a new
updated list of goals as well as how the blocks have been
reconfigured.

\begin{comment}
  To handle this task, we add additional machinery to our system in not
  only tracking people's current mental states, but also saving the
  mental states at certain points of significance. We define these
  points as being at when a person would begin to miss information as
  they leave the room, saving that full mental state to memory. In the
  case of $\humanb$, we define this saved state $p$ and is saved at step
  4 and would appear as it does in Figure 4. From here, the room does
  two things. The first is to determine how the goals of the room have
  changed and the second is how the world has minimally changed.
  To accomplish the first step, we generate a list of goal axioms from
  $\humanb$'s mental state and compare it against the room's current
  known goals, showing the goals that have been removed and added.
  The next step is determining how the configuration of the room has
  changed. To do this, we can employ Spectra our planner. We use the
  axioms that describe our configuration at $p$ as our initial state
  and the axioms at t to describe our goal state, and allow it to
  generate a plan on how we could have gotten there. The resulting
  plan is generated in around 848ms and shown back to the user where
  they see what changes, such as in figure \ref{fig:catch-up}), and
  allows them to update primarily what their beliefs in the goal of
  the system is (which the system saves in its understanding of
  $\humanb$'s updated mental state), and successfully completing
  this task.
\end{comment}


